SR+Codec: a Benchmark of Super-Resolution for Video Compression Bitrate Reduction

In recent years, there has been significant interest in Super-Resolution (SR), which focuses on generating a high-resolution image from a low-resolution input. Deep learning-based methods for super-resolution have been particularly popular and have shown impressive results on various benchmarks. However, research indicates that these methods may not perform as well on strongly compressed videos. We developed a super-resolution benchmark to analyze SR's capacity to upscale compressed videos. Our dataset employed video codecs based on five widely-used compression standards: H.264, H.265, H.266, AV1, and AVS3. We assessed 19 popular SR models using our benchmark and evaluated their ability to restore details and their susceptibility to compression artifacts. To get an accurate perceptual ranking of SR models, we conducted a crowd-sourced side-by-side comparison of their outputs. We found that some SR models, combined with compression, allow us to reduce the video bitrate without significant loss of quality. We also compared a range of image and video quality metrics with subjective scores to evaluate their accuracy on super-resolved compressed videos. The benchmark is publicly available at https://videoprocessing.ai/benchmarks/super-resolution-for-video-compression.html

==> inc/05-discussion.tex <==
\section{Discussion}
{\color{blue} In this section we discuss the limitations of our methodology and benchmark results.

\textbf{Downsample-based video codecs.} We do not add existing downscale-based video codecs to our benchmark because they usually use some additional features of the input video to aid the SR module after decompression. Not only it give these codecs a significant advantage over SR+codec pairs, it also contradicts the key idea of our benchmark to determine which SR architecture works best with each video codec standard.

\textbf{Speed of the SR methods.} In order to implement SR in a video codec you need SR to run in real time. Currently all SOTA SR methods are large models, so their speed on FullHD video is far from real-time. When we selected the models for the benchmark, we wanted to strike a balance between SRs that show the best quality and SRs that are close to real-time speed.}
